Adversarial Consistency and the Uniqueness of the Adversarial Bayes Classifier

Minimizing an adversarial surrogate risk is a common technique for learning robust classifiers. Prior work showed that convex surrogate losses are not statistically consistent in the adversarial context -- or in other words, a minimizing sequence of the adversarial surrogate risk will not necessarily minimize the adversarial classification error. We connect the consistency of adversarial surrogate losses to properties of minimizers to the adversarial classification risk, known as adversarial Bayes classifiers. Specifically, under reasonable distributional assumptions, a convex surrogate loss is statistically consistent for adversarial learning iff the adversarial Bayes classifier satisfies a certain notion of uniqueness.

==> Sections/9-acks.tex <==
%\begin{ack}
\section*{Acknowledgements}
Natalie Frank was supported in part by the Research Training Group in Modeling and Simulation
funded by the National Science Foundation via grant RTG/DMS – 1646339 and NSF grant DMS-2210583. Special thanks to Jonathan Niles-Weed for helpful conversations.
%\end{ack}

